Decoupling Strategy and Generation in Negotiation Dialogues

We consider negotiation settings in which two agents use natural language to bargain on goods. Agents need to decide on both high-level strategy (e.g., proposing \$50) and the execution of that strategy (e.g., generating "The bike is brand new. Selling for just \$50."). Recent work on negotiation trains neural models, but their end-to-end nature makes it hard to control their strategy, and reinforcement learning tends to lead to degenerate solutions. In this paper, we propose a modular approach based on coarse di- alogue acts (e.g., propose(price=50)) that decouples strategy and generation. We show that we can flexibly set the strategy using supervised learning, reinforcement learning, or domain-specific knowledge without degeneracy, while our retrieval-based generation can maintain context-awareness and produce diverse utterances. We test our approach on the recently proposed DEALORNODEAL game, and we also collect a richer dataset based on real items on Craigslist. Human evaluation shows that our systems achieve higher task success rate and more human-like negotiation behavior than previous approaches.

==> rl-bot-human-example.tex <==
\renewcommand{\bot}[1]{{\bf #1}}
\begin{table*}[ht]
{\footnotesize
\setlength\tabcolsep{0.5ex}
\begin{tabular}{p{8cm}l}
\toprule
\textbf{Title:} 1955 Chevy Belair   & \textbf{Listing Price:} \$16,000\\
\multicolumn{2}{l}{\textbf{Description:} 55 Chevy Belair, 2 door Sedan, Garaged over 25 years, California Car no rust. Extras: engines, transmission,}  \\
\multicolumn{2}{l}{fenders, hoods, grills to much to list.} \\
\midrule
\midrule
    (a) A: \rlword{length} (Buyer) \quad B: Human (Seller) &
    (b) A: \rlstate{length} (Buyer) \quad B: Human (Seller) \\
\midrule
    \begin{tabular}[t]{p{8cm}}
        A: \bot{hello} \\
        B: I am selling a 1955 Chevy Belair, were you interested? \\
        A: \bot{it's in good condition condition.} \\
        B: yes it's in good condition still \\
        A: \bot{it's in good condition condition.} \\
        B: It's been garaged for over 25 years, no rust, good engine,
        transmission, fenders, hood, grill. I'm asking \$16,000 \\
        A: \bot{i can do that low.} \\
        B: what's your offer? \\
        A: \bot{it's in good condition condition.} \\
        B: yes \\
        A: \bot{ok, that sounds good.} \\
    \end{tabular} &
    \begin{tabular}[t]{l}
        A: \bot{hi, is the 1955 Chevy Belair still available?} \\
        B: yes its been in a garage well maintained just like brand new \\
        A: \bot{what's the mileage on it?} \\
        B: under 100,000 \\
        A: \bot{nice. and the tires are all good?} \\
        B: yep yep all new transmissin no rust \\
        A: \bot{would you take 14720 for it?} \\
        B: if we could go to 1500 i could let it go for that \\
        A: \bot{that's still a little steep. what about 14720?} \\
        B: ok deal \\
        A: \bot{OFFER(\$14720)} \\
        B: ACCEPT
    \end{tabular} \\
\bottomrule
\end{tabular}
} % footnotesize
\caption{
    Example human-bot dialogue on \cl{} of RL models,
    where bot utterances are bolded.
    \rlword{length} devolved into degenerate behavior repeating itself while \rlstate{length} maintains coherency.
}
\label{tab:cl-human-rl-bot-chats}
\end{table*}

